Simulating thermal density operators with cluster expansions and tensor networks

We provide an efficient approximation for the exponential of a local operator in quantum spin systems using tensor-network representations of a cluster expansion. We benchmark this cluster tensor network operator (cluster TNO) for one-dimensional systems, and show that the approximation works well for large real- or imaginary-time steps. We use this formalism for representing the thermal density operator of a two-dimensional quantum spin system at a certain temperature as a single cluster TNO, which we can then contract by standard contraction methods for two-dimensional tensor networks. We apply this approach to the thermal phase transition of the transverse-field Ising model on the square lattice, and we find through a scaling analysis that the cluster-TNO approximation gives rise to a continuous phase transition in the correct universality class; by increasing the order of the cluster expansion we find good values of the critical point up to surprisingly low temperatures.

==> p6_numerics.tex <==
\section{Numerical Considerations}
\label{sec:numerics}

Some care has to be taken in order to construct numerically stable cluster expansions fast.


\subsubsection{Pseudoinversion}\label{pinv}

Constructing the unknown block(s) requires solving linear problems. This can generally be written in the following form after some bookkeeping
\begin{equation}
  A^1_{ I^1 \alpha^1 }   A^2_{ I^2 \alpha^2 }  \cdots  A^m_{ I^m \alpha^m }   X_{ \alpha^1  \alpha^2  \cdots \alpha^m j }  =  B_{  I_1  I_2 \cdots I_m   j }  .
\end{equation}
Here, $A^i$ are the different disconnected legs obtained by removing the unknown tensor(s). The legs $I^n$ groups all physical indices of the leg. The obvious choice is to solve a linear problem for all $A^i$ separately, but this causes numerical divergences because the problems are ill-conditioned due to their construction. Taking a pseudoinverse of all legs separately loses too much accuracy. Therefore the pseudoinverse of the full tensor $A = A^1 \otimes A^2 \otimes \cdots \otimes A^m$ is needed to obtain numerical stable and accurate cluster expansions. 

This can be implemented efficiently by performing an SVD decomposition on each leg first
\begin{equation}
    A^i = U^i \Sigma^i V^{i \dagger }
\end{equation}
with $U^i$ and $V^i$ unitary matrices and $\Sigma$ diagonal. $\Sigma = \Sigma^1 \otimes \Sigma^2 \otimes \cdots \otimes \Sigma^m$. The unitary matrices are trivial to invert, and the combined matrix $\Sigma$ is a sparse diagonal matrix. All diagonal entries of $\Sigma$ with $\sigma_i < \sigma_0$ are considered to be zero, the others are inverted. The threshold for inversion $\sigma_0$ is chosen as
\begin{equation}
    \sigma_0 = \alpha \cdot \max \left\{   \begin{array}{ll}
        \epsilon_{\text{machine}}  \\
        \max(  \epsilon_{B_i}  )
    \end{array} \right.
\end{equation}
with $\epsilon_{B_i}$ the error of all the smaller clusters $B_i$ which fit in the big cluster and $\alpha$ a prefactor. 

When the tensor X is a contraction of 2 tensors (e.g. \cref{4sitepatch}), an SVD decomposition is used to split them in 2 tensors.


%\subsubsection{Normalisation factor}
%The overal Pepo is normalised by a prefactor $ \alpha = | e^{ h_{12}/2 } |$. This is only important for imaginary time evolution. all calculations are done with a new prefactor $\alpha'$ that depends on the norm of the exact exponentiated Hamiltonian. 

\subsubsection{Symmetries}
The construction allows to include both lattice and internal symmetries.
\paragraph{lattice}
\textcolor{red}{Isotropy only implies this tensor can be made rotation invariant up to a gauge transformation}For an isotropic Hamiltonian on a square lattice, all blocks can be solved while imposing rotation symmetry over 90 degrees
\begin{equation}
    \pepob{Figures/2D/pepoSymA.pdf}{0.75} = \pepob{Figures/2D/pepoSymB.pdf}{0.75},
\end{equation}
For anisotrpic models, rotation symmetry over 180 degrees can still be imposed. This reduces the number of blocks that need to be solved significantly. Solving the blocks become a non-linear problem.

\paragraph{internal}
Global symmetries of the Hamiltonian can be used to speed up calculations with the resulting PEPO. 

\subsubsection{ Nonlinear problems }

There are 2 different places where non-linear problems appear in the construction of cluster expansions. First we focus on 
\begin{equation}\tag{\ref{tikzfig:plaquetter} revisited }
    \pepob{Figures/2D/pepoLoop.pdf} {0.75} .
\end{equation}
General methods for solving tensor rings are given in %\cite{Zhao2016}. 
In general, the smallest rank that solves the problem is unknown. In practice, $d^3$ seems sufficient. It is sufficient to iteratively solve each block with the techniques of \cref{pinv}. %The blocks should be scaled such that they have the same norm.

The linear solver can also be used to accurately calculate the corner piece of blocks such as
\begin{equation}\tag{ \ref{eq:loop_1ext}  revisited}
    \pepob{Figures/2D/pepoLoopExt.pdf}{0.75}  \; .
\end{equation}
Here, the other pieces of the loop are considered to be one leg $A^i$.

A second problem where a nonlinear problem shows up is when rotation symmetry is imposed.For example, \cref{5sitepatch} has 2 times the same tensor $O^{12}$ up to a rotation, and the simple loop \cref{tikzfig:plaquetter} even has 4 times the same tensor. This can be solved with a variational solver or by applying the linear solver sequentially. The variational solver can be sped up by computing the exact Jacobian from the network. The sequential solver calculates one the optimal tensor $O_{\text{new}}$ with on all the other sites $O_{\text{old}}$ and takes a step $\alpha$ in the right direction
\begin{equation}
    O_{\text{old}} \longleftarrow \alpha O_{\text{new}} + (1-\alpha)O_{\text{old}}
\end{equation}
 

\subsubsection{Region of convergence}

The convergence radius of the cluster expansions is limited to a certain inverse temperature $\beta$ or time t. Increasing the order of the cluster expansion does not improve upon the resulting error, and may lead to diverging cluster expansions. Another point where the convergence may fail is at the corner piece of the plaquette (cf \cref{eq:loop_1ext}) when the order of linear blocks is not high enough. The reason is that \cref{Tcond} is not fulfilled (for all types), as can easily be checked during construction.

%\begin{figure}.
%    \centering
%    \includegraphics[width=\linewidth]{Figures/Heis_ROC.pdf}
%    \caption{todo fix figure}
%    \label{fig:ROC}
%\end{figure}

% \subsubsection{Truncation}

% The bond dimension of a new block level scales as $d^N$, with $N$ the number of sites. This can be reduced with a truncated SVD to a given precision/ dimension. Higher order expansion can still be added, as long as the tolerance for the pseudoinverse $\sigma_0$ is chosen larger than the error introduced by the SVD.




